RTChoke: Efficient Real-Time Traffic Chokepoint Detection and Monitoring

We present a novel efficient adaptive sensing and monitoring solution for a system of mobile sensing devices that support traffic monitoring applications. We make a key observation that much of the variance in commute times arises at a few congestion hotspots, and a reliable estimate of congestion can be obtained by selectively monitoring congestion just at these hotspots. We design a smartphone application and a backend system that automatically identifies and monitors congestion hotspots. The solution has low resource footprint in terms of both battery usage on the sensing devices and the network bytes used for uploading data. When a user is not inside any hotspot zone, adaptive sampling conserves battery power and reduces network usage, while ensuring that any new hotspots can be effectively identified. Our results show that our application consumes 40- 80% less energy than a periodic sampling system for different routes in our experiments, with similar accuracy of congestion information. The system can be used for a variety of applications such as automatic congestion alerts to users approaching hotspots, reliable end-to-end commute time estimates and effective alternate route suggestions.

==> implementation.tex <==
\section{Implementation Details}
\label{sec:implementation}
We discuss the application- and server-side implementation details of \name{}.

\subsection{Application Implementation}
Our Android application is energy-aware in GPS sampling. We use low-energy sensors on the 
smart-phone for \textit{activity detection} to determine if the user is driving. If the user is driving, 
we turn on energy-efficient \textit{adaptive GPS sampling}. We now describe these processes.



\subsection{Server Implementation}
\label{sec:serverImpl}
The GPS values sampled by the users are transmitted to a central server where further analysis is
performed to detect hot-spots. This requires mapping GPS points to the road segments, computing the
speeds, and, finally, detecting congestion hot-spots.

%\subsubsection{Road Network Representation}
We use the data from Open Street Map (OSM) to model the underlying road network~\cite{osm}. OSM represents
the road network through a set of connected road-segments. Each segment (usually 100 to \unit{300}{m} in length).
% and multiple consecutive road-segments represents a complete road.
%Usually, each road-segment is around \unit{100-300}{m} in length.
Road-segments provides a fine-granular geo-spatial abstraction to map congestion information, since
each point on the segment have similar speeds.%can be expected to have correlation in speeds experienced by users.

\subsubsection{Trajectory Mapping and Speed Calculation}
We calculate the trajectory in which the vehicle is traveling using an existing map-matching algorithm~\cite{Newson2009}.
%This process requires fast spatial searching of road points near a given location, for which we utilize
%KD-Tree data structure~\cite{Samet1990}.
%The algorithm then uses a Hidden Markov Model to find the best matching trajectory for the samples.
We compute the approximate speeds that the vehicle has traveled by measuring the road-distance between two
consecutive GPS samples and the difference in the timestamp.
%Map-matching is a well-accepted methodology to calculate road trajectory taken by the vehicle by observing a
%stream of location samples. The algorithm is well-suited for GPS samples of the vehicle which are error-prone.
%The algorithm uses three phases for the right trajectory detection:
%\\\noindent\textit{1. Nearby Road-Segment Detection:} First, the algorithm detects the road-segments that are
%near (say, within \unit{100}{m}) to the GPS sample. These are the probable road-segments to map the vehicle's
%current position. This process requires spatial searching of road points near a given location. We utilize
%KD-Tree data structure (an efficient spatial data-structure) for fast searching of road points~\cite{Samet1990}.
%\\\noindent\textit{2. Computing emission probabilities:} This step computes the probability that the vehicle
%is on a road-segment for a given set of nearby road-segments. The probability is a function of the distance
%of the GPS sample from the road-segment. The distance is calculated by projecting an orthogonal point from
%sample point to point on road segment.
%\\\noindent\textit{3. Computing transmission probabilities:} This step utilizes the road-connectivity
%information to compute a probability that a vehicle is on road X given that the vehicle was probably on
%road Y during the last sample. This probability is dependent on number of factors such as road connectivity
%and shortest path between two points. For example, if the roads associated in the previous and current sample
%are unconnected (or the distance is unreasonably large to travel between the sampling times), then such
%points get weighted lower during this step -- even if such road-segments had larger weight during Step 2.
%
%Based on the above information of possible probabilities assigned to all road-segments for a sequence of
%samples, the algorithm uses a Hidden Markov Model to find the best matching trajectory for the samples.
%We compute the approximate speeds that the vehicle has traveled by measuring the road-distance between two
%consecutive GPS samples and the difference in the timestamp.

\subsubsection{Automatic Detection of Congestion Hot-Spots}


%Since each phone provides GPS samples using a bounded sampling interval, such incidents are guaranteed to
%detect low speeds due to incidences.
%
%Due to the bounded GPS sampling interval, each phone is guaranteed to provide multiple samples from the
%incident location, which can be used to detect congestion at the server side. Maximum GPS sampling interval
%is set based on the user-specified power budget, however we make sure to not set it very high. Note that if
%%the congestion situation is alleviated in the duration less than the maximum GPS sampling interval, then it
%is more likely not a congestion hot-spot, and thus can be ignored.

%\paragraph{Automatic detection of congestion hot-spots}
%When the server receives real-time updates about users' locations, it filters the erroneous GPS samples and stores them into a spatio-temporal data structure. Essentially, we construct a graph for the whole road-network, where a vertex of the graph represents a road-segment from the OSM data. Each user's location data is mapped to its corresponding road-segment. For each road-segment, we also maintain time-ordered bins for temporal analysis.
%
%{\bf Defining a congestion hot-spot:}
%Different approaches exist to classify a road-segment is a congestion hot-spot, however majority of them rely on parameters such as maximum-speed limit on a road, number of lanes, or maximum density of cars on a road-segment~\cite{kerner2004recognition}. While such parameters are easily available for roads in developed countries, they are either not defined or changing over time or not followed well in the developing countries. Thus, to detect congestion hot-spots, we do not assume the knowledge of these parameters. Instead, we use average speed to define different levels of congestion. Owing to the terminology from the literature~\cite{kerner2004three}, we categorize hot-spots using low-, medium-, and high-congestion levels.
%
%{\bf Incident based congestion detection:}
%Due to the bounded GPS sampling interval, each phone is guaranteed to provide multiple samples from the incident location, which can be used to detect congestion at the server side. Maximum GPS sampling interval is set based on the user-specified power budget, however we make sure to not set it very high. Note that if the congestion situation is alleviated in the duration less than the maximum GPS sampling interval, then it is more likely not a congestion hot-spot and thus can be ignored.
%
%{\bf Separating hot-spots from low-speed roads:}
%Different roads may have different speed signatures depending on the road size and road-surface conditions such as speed-bumps, potholes, etc. Thus, low average speeds do not necessarily mean a congestion hot-spot. Therefore it is important differentiate between lower average speeds due to congestion hot-spots vs. that due to road-conditions.
%
%We propose an approach to set different threshold values for average speeds for different road-segments. Essentially, for each road-segment, we keep track of the maximum speed, $V_{max}$, observed for any vehicle over history. Based on $V_{max}$, we set thresholds for different congestion levels. We set $\frac{1}{4} \frac{V_{max}}{2}$ as a threshold for high-congestion, $\frac{1}{2} \frac{V_{max}}{2}$ for medium-congestion, and $\frac{3}{4} \frac{V_{max}}{2}$ for low-congestion levels. We note that a different thresholding mechanism can also be devised based on data with ground-truth.

